FAAC: Facial Animation Generation with Anchor Frame and Conditional Control for Superior Fidelity and Editability

Over recent years, diffusion models have facilitated significant advancements in video generation. Yet, the creation of face-related videos still confronts issues such as low facial fidelity, lack of frame consistency, limited editability and uncontrollable human poses. To address these challenges, we introduce a facial animation generation method that enhances both face identity fidelity and editing capabilities while ensuring frame consistency. This approach incorporates the concept of an anchor frame to counteract the degradation of generative ability in original text-to-image models when incorporating a motion module. We propose two strategies towards this objective: training-free and training-based anchor frame methods. Our method's efficacy has been validated on multiple representative DreamBooth and LoRA models, delivering substantial improvements over the original outcomes in terms of facial fidelity, text-to-image editability, and video motion. Moreover, we introduce conditional control using a 3D parametric face model to capture accurate facial movements and expressions. This solution augments the creative possibilities for facial animation generation through the integration of multiple control signals. For additional samples, please visit https://paper-faac.github.io/.

==> sec/3_finalcopy.tex <==
\section{Final copy}

% % You must include your signed IEEE copyright release form when you submit your finished paper.
% % We MUST have this form before your paper can be published in the proceedings.

% % Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

==> sec/combination_figure.tex <==
\newcommand{\newteasercombination}{
  %\vspace{-1em}
	\centering
	\includegraphics[width=1.00\textwidth, trim=0em 0em 0em 0em, clip]{imgs/combination.png}
    \vspace{-2em}
  \captionof{Pose and Expression Combination
  \vspace{-1em}
  }
	\label{fig:combination}
  \vspace{1.5em}
}

==> sec/method_figure.tex <==
\newcommand{\newteasermethod}{
  %\vspace{-1em}
	\centering
	\includegraphics[width=1.00\textwidth, trim=0em 0em 0em 0em, clip]{imgs/method_faac.png}
    \vspace{-2em}
  \captionof{figure}{\textbf{Overview.} We propose a training method and an inference method for facial video generation. During training, we freeze the T2I model and train the Temporal attention Module with the help of our Anchor Frame mechanism. During inference, coherent video samples can be generated simply with our Anchor Frame Inference to get the same editability and fidelity of the original T2I model by the training-free or training-based approach.
  \vspace{-1em}
  }
	\label{fig:teaser_method}
  \vspace{1.5em}
}
